Meta Learning in the Continuous Time Limit

In this paper, we establish the ordinary differential equation (ODE) that underlies the training dynamics of Model-Agnostic Meta-Learning (MAML). Our continuous-time limit view of the process eliminates the influence of the manually chosen step size of gradient descent and includes the existing gradient descent training algorithm as a special case that results from a specific discretization. We show that the MAML ODE enjoys a linear convergence rate to an approximate stationary point of the MAML loss function for strongly convex task losses, even when the corresponding MAML loss is non-convex. Moreover, through the analysis of the MAML ODE, we propose a new BI-MAML training algorithm that significantly reduces the computational burden associated with existing MAML training methods. To complement our theoretical findings, we perform empirical experiments to showcase the superiority of our proposed methods with respect to the existing work.

==> Meta Learning_arXiv version 2.0/experiments.tex <==
\section{Numerical Experiments}\label{sec:experiments}

Our experiments evaluate the \bmm algorithm proposed in \cref{sec:main-results} against the \maml algorithm on a series of learning problems. More specifically, we compare both methods on two different tasks: linear regression and binary classification with a Support Vector Machine (\svm). They correspond to two different types of task loss $f_i$: strongly convex and convex. For both types of problem we compare the methods on both synthetic and real data.

\paragraph{Linear regression.} For the linear regression problem with synthetic data, we meta-learn the model parameter $\gamma\in\Rd$ from a set of generated data that correspond to $M = 10$ individual linear regression tasks, each with dimension $d = 20$. A ground truth vector $\gamma_i\in\Rd$ is generated independently for each individual task. Each $\gamma_i$ has its coordinates drawn from i.i.d.\ standard normal distributions. From each task, we generate $n = 100$ training samples $\{x_j,y_j\}\in\Rd\times\RR$, where each entry of $x_j$ is subject to an i.i.d.\ standard normal distribution and $y_j = x_j\transpose\gamma_i + \sigma Z_j$ where $Z_j$ is a standard normal variable and $\sigma = 1$ in our case. We also initialize the model parameter $\gamma\in\Rd$ randomly in the way we generate $\gamma_i$, and the \maml step size $\alpha = 0.3$ is fixed for all tasks. Each linear regression task $i$ has a strongly convex loss function $f_i(\gamma) = \|y - X\gamma\|^2$, where $X = [x_1,\ldots,x_n]\transpose$ and $y = [y_1,\ldots,y_n]\transpose$. We take the gradient descent step size $\beta = 0.05$ for both \bmm and \maml, and we present the numerical results in \cref{fig:lr_function,fig:lr_gradient}. 
For the linear regression problem on the \texttt{Diabetes} data set, we divide the original data into $M = 4$ tasks with dimension $d = 8$ according to male/female and whether the person is older than mean age of the data. We initialize the model parameter $\beta$ randomly with i.i.d.\ normal entries, and the \maml step size $\alpha = 0.5$ is fixed for all tasks. We choose $\beta = 0.1$ and run the algorithms. Numerical results are presented in \cref{fig:lr-diabetes-function,fig:lr-diabetes-gradient}.
Compared to \maml, our \bmm algorithm in \cref{fig:lr_function} converges to a neighborhood of stationary point of $F$ in 25 steps, where \maml is far from convergence. After 50 iterations, \bmm also shows its superiority in computational efficiency over \maml by having 37\% and 36\% decrease in computation time on synthetic and real data, respectively.

\paragraph{Support vector machine.} For binary classification with an \svm, we meta-learn from $M = 50$ binary classification tasks in $d = 20$ dimensional space, where each one of the individual tasks is composed of $n = 300$ samples $\{x_j,y_j\}\in\Rd\times\{\pm 1\}$, evenly split between the positive and negative classes. We generate these training data sets with the default data generating function from \texttt{scikit-learn}. For each task $i$, it is equipped with a convex (but not strongly convex) hinge loss $f_i(w) = \ReLu(y - X w)$, where $X = [x_1,\ldots,x_n]\transpose$ and $y = [y_1,\ldots,y_n]\transpose$. During the experiment, we take the \maml parameter $\alpha = 0.3$ for all tasks, and the gradient descent step size $\beta = 0.1$ is used for both the \bmm and the \maml. The corresponding numerical results are presented in \cref{fig:svm_function,fig:svm_gradient}. 
For the binary classification on \texttt{MNIST}, we design $M = 5$ tasks, each to be a classification on different digits (classify $1,3,5,7,9$ against $2,4,6,8,0$), which has dimension $d = 784$. Each task has $n = 200$ samples, and the \maml parameter $\alpha = 0.3$ is fixed for all tasks. We take $\beta = 0.01$ for the experiment, and the result is reported in \cref{fig:svm-mnist-function,fig:svm-mnist-gradient}.
Compared to \maml, our \bmm algorithm in \cref{fig:svm_gradient} reaches the region with small gradient norm $\|\nabla F(w)\|$ in less than 30 steps, where \maml still has a much larger gradient. In these experiments, \bmm shows its superiority in computational efficiency over \maml by having a 19\% and 37\% decrease in computation time on the synthetic and real data, respectively.


\begin{figure}[ht]
\centering

\begin{subfigure}[b]{.242\textwidth}
  \centering
  \includegraphics[width=\linewidth]{lr_function}
  \caption{Linear regression on synthetic data}
  \label{fig:lr_function}
\end{subfigure}\hfill
\begin{subfigure}[b]{.242\textwidth}
  \centering
  \includegraphics[width=\linewidth]{lr_diabetes_function}
  \caption{Linear regression on \texttt{Diabetes}}
  \label{fig:lr-diabetes-function}
\end{subfigure}\hfill
\begin{subfigure}[b]{.242\textwidth}
  \centering
  \includegraphics[width=\linewidth]{svm_function}
  \caption{Binary class.~with \svm on synthetic data}
  \label{fig:svm_function}
\end{subfigure}\hfill
\begin{subfigure}[b]{.242\textwidth}
  \centering
  \includegraphics[width=\linewidth]{mnist_svm_function}
  \caption{Binary classification with \svm on \texttt{MNIST}}
  \label{fig:svm-mnist-function}
\end{subfigure}

\medskip

\begin{subfigure}[b]{.242\textwidth}
  \centering
  \includegraphics[width=\linewidth]{lr_gradient}
  \caption{Linear regression on synthetic data}
  \label{fig:lr_gradient}
\end{subfigure}\hfill
\begin{subfigure}[b]{.242\textwidth}
  \centering
  \includegraphics[width=\linewidth]{lr_diabetes_gradient}
  \caption{Linear regression on \texttt{Diabetes}}
  \label{fig:lr-diabetes-gradient}
\end{subfigure}
\begin{subfigure}[b]{.242\textwidth}
  \centering
  \includegraphics[width=\linewidth]{svm_gradient}
  \caption{Binary class.~with \svm on synthetic data}
  \label{fig:svm_gradient}
\end{subfigure}\hfill
\begin{subfigure}[b]{.242\textwidth}
  \centering
  \includegraphics[width=\linewidth]{mnist_svm_gradient}
  \caption{Binary classification with \svm on \texttt{MNIST}}
  \label{fig:svm-mnist-gradient}
\end{subfigure}
\caption{Comparisons on the performance of \bmm versus \maml on linear regression and binary classification with \svm. The figures on the first row compare the \bmm and \maml with function values on the \maml loss $F(w_k)$ at each iteration $k$. The figures in the second row show the trajectory of the corresponding gradient norm values evaluated at every iteration $k$. The blue lines represent the performance on \bmm, and the red lines represent that on \maml. }
\label{fig:images}
\end{figure}

It is noteworthy that even if our method only provably works for strongly convex loss functions $f_i$, it empirically achieves good performance on real world data for many strongly convex and even convex loss functions, such as \svm. 
We remark that the gradient norm for the \bmm shown in \cref{fig:lr_gradient,fig:svm_gradient,fig:svm-mnist-gradient,fig:lr-diabetes-gradient} represents different quantities in different stages of the algorithm. Specifically, it denotes $\|\nabla F(w_k)\|$ when the \bmm descends on $F$ at the \kth iteration; analogously, it represents $\|\nabla f(w_k)\|$ when the \bmm descends on $f$. The jumps in \cref{fig:svm_gradient,fig:svm-mnist-gradient,fig:svm-mnist-function} show clearly the transitions between two phases.


==> Meta Learning_arXiv version 2.0/introduction.tex <==
\section{Introduction}\label{sec:intro}

In machine learning, an ideal learner is able to speed up the learning of new tasks based upon previous experiences. This goal has been shared among different but highly related approaches such as  few-shot learning \citep{snell2017prototypical}, domain adaptation~\citep{yu2018one,li2018learning}, transfer learning \citep{pan2009survey}, and meta  learning (\aka \emph{learning to learn}) ~\citep{thrun2012learning,naik1992meta,schmidhuber1987evolutionary,hochreiter2001learning}. In particular,  meta-learning addresses a general optimization framework that aims to learn a model based on data from previous tasks, so that the learned model, after fine-tuning, can adapt to and perform well on new tasks. This idea has been successfully applied to different learning scenarios including reinforcement learning ~\citep{wang2016learning,duan2016rl,schweighofer2003meta}, deep probabilistic models~\citep{edwards2016towards,lacoste2017deep,grant2018recasting}, language models~\citep{radford2019language}, imitation learning~\citep{duan2017one}, and unsupervised learning~\citep{hsu2018unsupervised}, to name a few.  Previous works have also investigated meta learning  from a variety of perspectives and methods, including memory-based neural networks~\citep{santoro2016meta,munkhdalai2017meta}, black-box optimization ~\citep{duan2016rl,wang2016learning1}, learning to design an optimization algorithm~\citep{andrychowicz2016learning},  attention-based models~\citep{vinyals2016matching}, and LSTM-based learners~\citep{ravi2016optimization}. 

One of the gradient-based meta-learning algorithms that has been widely used and enjoys great empirical successes is the \emph{model-agnostic meta-learning} proposed in \citep{Finn2017}. 
Rather than minimizing directly on a combination of task losses, \maml meta-trains by minimizing the loss evaluated at one or multiple gradient descent steps further ahead for each task. The intuition is as follows: First, this meta-trained initialization resides close to the best parameters of all training tasks. Second, for each new task, the model can then be easily fine-tuned for that specific new task with only a small number of gradient descent steps. 
Following this work, many experimental and theoretical studies of \maml have been carried out~\citep{song2019maml,behl2019alpha,grant2018recasting,yang2019norml,rajeswaran2019meta}. In particular, \citet{fallah2019convergence} and \citet{mendonca2019guided} investigated the convergence of \maml to first order stationary points. Moreover, \citet{finn2019online} studied an online variant of \maml and \citet{antoniou2018train} proposed various modifications to \maml to improve its performance.  Empirically, \citet{raghu2019rapid} found that the success of \maml can be primarily associated to feature reuse, given high quality representations provided by the meta-initialization. 


\maml assumes a shared parameter space $\Rd$ among all the tasks and learns an initialization $\widehat w\in\Rd$ from a batch of tasks at \emph{meta-learning} time, such that performing a few steps of gradient descent from this initialization at \emph{meta-testing} time minimizes the loss function for a new task on a smaller dataset. More specifically, in a task pool with total $M$ candidate tasks,  each task $\calT_i$ is sampled from the pool according to a distribution $p(\calT)$ and has a corresponding risk function $f_i:\Rd\to\RR$ that is parameterized by a shared variable $w\in\Rd$. This function measures the performance of the parameter $w$ on task $\calT_i$. In practice we estimate this risk function from a set of training data for each task. However, for simplicity, we directly work with the risk function in this paper and assume that we can acquire the knowledge of the task loss $f_i$ from an oracle. At meta-learning time, \maml looks for a warm start $\widehat w$ via solving an optimization problem that minimizes the expected loss over $f_i$ after one step of gradient descent, \ie,
\begin{align}\label{eqn:maml-opt}
    \widehat w = \argmin_w \expect_{i\sim p}[f_i(w - \alpha\nabla f_i(w))],
\end{align}
where $\expect_{i\sim p}$ denotes the expectation over sampled tasks and $\alpha$ represents the \maml step size (also referred to as the \maml parameter).
To ease the burden on notation, we define the \maml loss function of task $\calT_i$ to be $F_i(w) \defeq f_i(w - \alpha\nabla f_i(w))$. Further, we define some shorthand for the expected loss $f(w) \defeq \expect_{i\sim p}f_i(w)$ and the expected \maml loss $F(w) \defeq \expect_{i\sim p}F_i(w)$. Now we are able to represent the optimization problem \eqref{eqn:maml-opt} in a more concise form: $\argmin_w F(w)$.

Solving \eqref{eqn:maml-opt} yields a solution $\widehat w$ that in expectation serves as a good initialization point, such that after a step of gradient descent it achieves the best average performance over all possible tasks. However, because the objective function $F(w)$ is non-convex in general, there is no guarantee that one is able to find a global minimum. Therefore it is common to instead consider finding an approximate stationary point $\widehat w$ where $\|\nabla F(\widehat w)\| \leq \varepsilon$ for some small $\varepsilon$ \citep{fallah2019convergence}.




In this paper, we study the \maml algorithm proposed in \citep{Finn2017}, in which \maml meta-learns the model by performing gradient descent on the \maml loss. We begin by establishing a smooth approximation of this discrete-time iterative procedure and considering the continuous-time limit by taking an infinitesimally small step size. With any initialization of the parameter, the problem is transformed into an \emph{initial value problem} (\ivp) of an \ode, which is the underlying dynamic that governs the training of a \maml model. Specifically, We consider the convergence of the gradient norm $\|\nabla F(w)\|$ and the function value $F(w)$ under the continuous-time limit of \maml.


Our contributions can be summarized as follows:
\begin{itemize}
    \item
    We propose an \ode that underlies the training dynamics of a \maml model. In this manner, we eliminate the influence of the manually chosen step size. %
    The algorithm in \citep{Finn2017} can be viewed as an forward Euler integration of this \ode.
    \item 
    We prove that the aforementioned \ode enjoys a linear convergence rate to an approximate stationary point of $F$ for strongly convex task losses. In particular, it achieves an improved convergence rate of $\calO(\log\frac{1}{\varepsilon})$, compared to $\calO(\frac{1}{\varepsilon^2})$ in \citep{fallah2019convergence}. Note that the \maml loss $F$ may not be convex even if the individual task losses $f_i$ are strongly convex.
    \item
    We show that for strongly convex task losses with moderate regularization conditions, the \maml loss $F$ has a unique critical point that is also the global minimum.
    \item 
    We propose a new algorithm named \bmm for strongly convex task losses that is   computationally efficient and enjoys a similar linear convergence rate to the global minimum compared to the original \maml. It also converges significantly faster than \maml on a variety of learning tasks.
\end{itemize}





